Capture the Flag for Team Construction in Cybersecurity

Team collaboration among individuals with diverse sets of expertise and skills is essential for solving complex problems. As part of an interdisciplinary effort, we studied the effects of Capture the Flag (CTF) game, a popular and engaging education/training tool in cybersecurity and engineering, in enhancing team construction and collaboration. We developed a framework to incorporate CTF as part of a computer-human process for expertise recognition and role assignment and evaluated and tested its effectiveness through a study with cybersecurity students enrolled in a Virtual Teams course. In our computer-human process framework, the post-CTF algorithm using the CTF outcomes assembles the team (assigning individuals to teams) and provides the initial role assignments, which then gets updated by human-based team discussions. This paper shares our insights, design choices/rationales, and analyses of our CTF-incorporated computer-human process framework. The students' evaluations revealed that the computer-human process framework was helpful in learning about their team members' backgrounds and expertise and assigning roles accordingly made a positive impact on the learning outcomes for the team collaboration skills in the course. This experience report showcases the utility of CTF as a tool for expertise recognition and role assignments in teams and highlights the complementary roles of CTF-based and discussion-based processes for an effective team collaboration among engineering students.

==> CTF_Team_Discussions.tex <==

\subsection{Discussions and Considerations for CTF Framework Implementation}
\syc{Need revision; Probably would be moved to the Conclusion section or incorporated earlier}
Our implementation is efficient, i.e., solves in polynomial time O($m$) for team assembly and O($m^4$) for role assignment, provides a reasonably good solution based on our solution selection criteria in Section~\ref{subsec:solution_selection}, and is appropriate for our team construction for the Virtual Teams Course for the cybersecurity students. Future work can include: further optimization and complexity analyses for team assembly in Section~\ref{subsec:team_assembly} and for role assignment in Section~\ref{subsec:role_assignment} (for example, a joint optimization between team assembly and role assignment may be NP-hard to find the solution and require a suboptimal but practical heuristic approach, e.g., greedy algorithm), the generality analyses for the assumptions and rules in Section~\ref{subsec:solution_feasibility} (to establish a model using our framework in different team construction scenarios), and the metric adjustment for the solution selection in Section~\ref{subsec:solution_selection} (e.g., there can be other team construction scenarios prioritizing one team over the other as opposed to making them even/fair). 
\syc{Also include using more data and list the additional data in the current CTF which could have helped, e.g., number of trials and failures in each role categories to determine their interests}

==> CTF_validation.tex <==
%\sw{Plots, 10 page limit, be compact}
%By simulating random team assemblies, we find that the group 1 and group 2 scores diverge towards 1332.75.

\begin{figure}
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{BarPlotAlgorithms_capacity.pdf}
  \caption{Team Assembly Capacity}
  \label{fig:sub2}
\end{subfigure}
\quad
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{BarPlotAlgorithms_sd.pdf}
  \caption{Standard deviation across the team members within team \syc{This seems counter-intuitive; was expecting our approach to have small S.D.}}
  \label{fig:sub2}
\end{subfigure}
\quad
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{BarPlotAlgorithms_score.pdf}
  \caption{Role Assignment Score}
  \label{fig:sub1}
\end{subfigure}%
% \begin{subfigure}
% \centering
% \includegraphics[]
% \end{subfigure}
\caption{}
\label{fig:test}
\end{figure}

% \begin{table*}[tp]
% \begin{tabular}{lllll}
%                   & \begin{tabular}[c]{@{}l@{}}$N_1$ Team Assembly\\ Capacity\end{tabular} & \begin{tabular}[c]{@{}l@{}}$N_2$ Team Assembly\\ Capacity\end{tabular} & \begin{tabular}[c]{@{}l@{}}$N_1$ Role Assignment\\ Hungarian Score\end{tabular} & \begin{tabular}[c]{@{}l@{}}$N_2$ Role Assignment\\ Hungarian Score\end{tabular} \\ \hline
% Random selection   & 2665.5 ($\sigma=324.97$) & 2665.5 ($\sigma=324.97$) & 875.18 ($\sigma=123.33$) & 875.18 ($\sigma=123.33$) \\ \hline
% Our approach      & 2721                  & 2610                  & 989         & 797         \\ \hline
% Exhaustive maximum & 3509                  & 1822                  & 1150                  & 1150                  \\ \hline
% \end{tabular}
% \caption{Comparison between the three algorithms in both team assembly and role assignment. The random selection method runs a Monte Carlo simulation to find the convergence of randomly selecting $\vec{s'}$ which is then input into the optimal role assignment. By default, $\sigma=0$ unless otherwise stated.}
% \label{tab:assignment_scores}
% \end{table*}


\begin{table}[]
\begin{tabular}{ccccccc}
                        & $N_1$ Capacity & $N_2$ Capacity & $N_1$ $\sigma$ & $N_2$ $\sigma$ & $N_1$ Team Score & $N_2$ Team Score \\ \hline
Random                  & 2665.5          & 2665.5          & 180.18               & 180.18               & 875.18  & 875.18  \\ \hline
Our approach            & 2721            & 2610            & 191.52               & 197.76               & 989          & 797          \\ \hline
Max Capacity for Team 1 & 3509            & 1822            & 75.3               & 115.95               & 1150         & 598          \\ \hline
\end{tabular}
\caption{Comparison between the three algorithms in both team assembly and role assignment. The random selection method runs a Monte Carlo simulation to find the convergence of randomly selecting $\vec{s'}$ which is then input into the optimal role assignment. By default, $\sigma=0$ unless otherwise stated.}
\label{tab:assignment_scores}
\end{table}


% \begin{table*}[tp]
% \begin{tabular}{ l l l l }
%                   & \begin{tabular}[c]{@{}l@{}}Team Capacity\end{tabular} & \begin{tabular}[c]{@{}l@{}} Team Score \end{tabular} & \begin{tabular}[c]{@{}l@{}} Standard Deviation \\ \hline
% Random Selection    & 2665.5     & 875.18   & XXX \\ \hline
% Our approach (Team 1)      & 2721                  & 989                  & XXX         \\ \hline
% Our approach (Team 2)      & 2610                  & 797                  & XXX         \\ \hline
% Max Capacity for Team 1 (Team 1) & 3509                  & 1150                  & XXX                  \\ \hline
% Max Capacity for Team 1 (Team 2) & 1822                  & XXX                  & XXX                  \\ \hline
% \end{tabular}
% \caption{Comparison between Our Approach vs. Random Selection vs. Max Capacity for Team 1. The estimations for Random Selection is averaged across the possible team assembly cases, 
% and the standard deviation is across the team members within a team.}
% \label{tab:assignment_scores}
% \end{table*}



\subsection{Comparison with Other Team Assembly Algorithms}
\label{subsec:ctf_assembly_comparison}

In Section~\ref{subsec:CTF_implementation_rules}, while we have a clear definitions for optimization for role assignment to maximize the team score to maximize the aggregate scores/contributions for a team, our definition for ``optimal'' is not well-defined and incorporates a tradeoff between increasing the team capacity and decreasing the spread/discrepancies across the team members within a team. Therefore, we compare our approach with two alternative algorithms, which are \emph{Random Selection} and \emph{Max Capacity for Team 1} 
\syc{To self: Need to continue from here}



%\section{Validations and Assessments}

\subsection{CTF Validations \syc{CTF Analyses}}
\label{sec:validations}

In this section, we look into the validation metrics for the team assembly and role assignment. By comparing our results to the brute force of each assignment we can determine how close our algorithm is to the optimal algorithm. The optimal brute force algorithm operates in exponential time complexity, O($2^n$) for team assembly, and O($n!$) for role assignment, thus, we can only compare our results to the optimal solution for small numbers of $p$, $r$. We assume two teams of five members each ($p=10$), and the five roles ($r=5$) of $\mathcal{R}$ = \{ IN, DE, AN, IM, CO \}.
%\syc{Simeon: Let's assume two teams ($n=2$), of five members each, and the five roles  ($r=5$) of $\mathcal{R}$ = \{ IN, DE, AN, IM, CO \}.}

\subsubsection{CTF-Based Team Assembly}
Due to the strategy in selecting teams to optimize the fairness in skills, our CTF-based team assembly provides a better outcome when compared to a random team selection and assembly. To quantify this, we simulate the random team assembly process and compare the outcome with our work as well as the optimal exhaustive case.

A team assembly matrix, $\vec{s'}$, can be represented in compact binary notation where the $i$'th index $\vec{s'}$ refers to player $\mathcal{P}_i$ with a Boolean value (e.g. 0 or 1) refering to the participant's group assignment. For example, assignment $992=1111100000$ means that $p_1$ through $p_5$ will be assigned to group 2, and $p_6$ through $p_{10}$ will be assigned to group 1. With this definition, an exhaustive search will take O($2^n$), however, by adding the additional constraint in which the number of $1$'s and $0$'s must have no difference greater than 1, i.e. the number of groups, $n$, must be enforced where every team has the same cardinality. This eliminates assignments such as $\vec{s'}_i=512$ because the number of 1s and 0s are imbalanced.


%\sw{Average bar and standard deviation bar, our scheme = 0, random, exhaustive}
Table~\ref{tab:assignment_scores} compares these three approaches in the team assembly as well as the outcome scores after the role assignment is done.
The team-aggregate score for our algorithm across all elements in the 5x5 matrices, \sw{$N_1$ and $N_2$} is 989 and 797, respectively.
When comparing this to the average case in which a random team assignment is made by selecting a random integer between $0$ and $2^p$ and interpreting the binary notation as an assembly mapping, we find that the team-aggregate scores diverge towards 666.38 for both $N_1$ and $N_2$. Thus, our team assembly algorithm yields a 25.37\% increase in score utilization.
The exhaustive algorithm which operates in exponential time yields a result of $N_1=1063$ and $N_2=747$, which is only 1.33\% more efficient than our approach, which operates in linear time.

%Maximum difference between team members in row-aggregate score

%\syc{Simeon: How is the CTF-based team assembly more fair than the random team assembly? Quantify the fairness gain, for example, find the average aggregate scores for the random team assembly cases.}
%\syc{Simeon: Let's measure: i) the team-aggregate score across all the elements in the 5x5 matrix and ii) the *maximum* difference between the team members in the row-aggregate score (i.e., the row-aggregate score difference between the best member vs. the worst member). Output these measurements for all possible cases when doing the brute-force/exhaustive search so that we can later compute the averages and the max for these measurements.}

\subsubsection{CTF-Based Initial Role Assignment}
Similar to the team assembly, we compare the initial role assignment across to random selection, our approach, and exhaustive maximum. Our CTF role assignment when compared to the random role assignment and exhaustive role assignment show significant variation between performances and scores. For role assignment, we use the Hungarian algorithm in all three approaches, and compare the corresponsing scores. %Table~\ref{tab:assignment_scores}

%Our CTF role assignment is done in two ways: 1) using the Hungarian algorithm, and 2) using an exhaustive search. We also include a random role assignment case in which the roles for each team are distributed to each team member randomly. Finally, we quantify a joint team assembly and role assignment where we use the Hungarian algorithm to distribute each role assignment for every exhaustive permutation of team assembly/grouping arrangements.
\syc{Simeon: Compare the CTF role assignment vs. the random role assignments. Quantify the aggregate-score for CTF vs. random (the average in this random assignment case) vs. the joint assembly/assignment. The last joint case corresponds to "jointly conducting the initial role assignment by assigning the role at the time the participant gets selected for the team so that the participant's highest-scoring role becomes his/her role" in Section~\ref{subsec:team_assembly}.}

\syc{Simeon: Let's fix the team assembly based on our discussion after swapping Derek and Noah. Let's measure: the team-aggregate score while greying/zeroing out the non-colored cells (so only focus on the colored cell corresponding to the selected member-role combination). Output these measurements for all possible cases when doing the brute-force/exhaustive search so that we can compute the average case when choosing the initial role assignment randomly.}

